Optimal Non-Uniform Mapping for Probabilistic Shaping

The construction of optimal non-uniform mappings for discrete input memoryless channels (DIMCs) is investigated. An efficient algorithm to find optimal mappings is proposed and the rate by which a target distribution is approached is investigated. The results are applied to non-uniform mappings for additive white Gaussian noise (AWGN) channels with finite signal constellations. The mappings found by the proposed methods outperform those obtained via a central limit theorem approach as suggested in the literature.

==> Makefile <==
PROJECT=many
TMPFILES=*.aux *.bak *.bbl *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps\
*.ind *.idx *.ilg *.gls *.glo *.glg *.acn *.acr *.alg *.ist *.out\
*.thm
ARXIVTMP=*.aux *.bak *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps $(PROJECT).pdf *.bib .*.xml


default:
	pdflatex -shell-escape $(PROJECT).tex;

clean:
	rm -f $(TMPFILES);

clean_pdf:
	rm -f $(PROJECT).pdf;

final: clean clean_pdf
	pdflatex -shell-escape $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
	bibtex $(PROJECT);
	pdflatex $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
arxiv:
	rm -f $(ARXIVTMP);
	rm -rf .git;



==> figures/problem.tex <==
\section{Problem Statement}
\label{sec:quantization}
\begin{figure}
\centering
\footnotesize
\def\svgwidth{1.0\columnwidth}
\includesvg{figures/quantization}
\caption{Example for quantization as defined in \eqref{eq:quantization}. First, the left-open interval $(0,1]$ is partitioned into $M=4$ left-open uniform intervals of length $1/M$. Second, the interval $(0,1]$ is partitioned into left-open intervals whose lengths are the probabilities of the target pmf. Finally, the approximation of $t_i$ is determined by the number of uniform intervals whose middle points lie within the interval that corresponds to $t_i$. Thus, the quantization of $\vect^T=(0.16,\;0.62,\;0.22)^T$ is $\vecd^T=\frac{1}{4}(1,\;2,\;1)^T$.
}
\label{fig:quantization}
\end{figure}
\subsection{Quantization}
The \emph{cumulative distribution function} (cdf) $\boldsymbol{T}$ for the target pmf $\vect$ is defined  by
\begin{align}
T_i = \sum_{k=1}^i t_k,\quad i=1,\dotsc,n.
\end{align}
The $i$th entry of the $M$-type approximation by quantizing $\vect$ is given by
\begin{align}
d_i = \frac{1}{M}\cdot\left|\left\{\ell\in\setz\colon T_{i-1}<\frac{\ell-\frac{1}{2}}{M}\leq T_i\right\}\right|\label{eq:quantization}
\end{align}
where $\setz$ denotes the set of integers and $|\cdot|$ the cardinality of a set. We define $T_0=0$. An illustrating example is displayed in Fig.~\ref{fig:quantization}. Note that if $t_i=0$, then $T_{i-1}=T_i$, which implies that the set on the right hand side of \eqref{eq:quantization} is empty. Consequently, we have
\begin{align}
t_i=0\quad\Rightarrow\quad d_i = 0.\label{eq:probZero}
\end{align}
We make use of \eqref{eq:probZero} later. For each $i$, $d_i$ is bounded by
\begin{align}
t_i-\frac{1}{M}\leq d_i\leq t_i+\frac{1}{M}\label{eq:quantBounds}
\end{align}
which implies
\begin{align}
|t_i-d_i|\leq\frac{1}{M}.
\end{align}
This observation immediately gives the following proposition.
\begin{proposition}\label{prop:general}
Let $f$ be a continuous function from the set of pmfs with $n$ entries to the set of real numbers. Then a target pmf $\vect$ can be approximated arbitrarily well by an $M$-type pmf in the sense that for any $\epsilon>0$, there is an $M_0$, such that for all $M>M_0$ we have $|f(\vect)-f(\vecd_M)|<\epsilon$ where $\vecd_M$ is the $M$-type pmf found by quantizing $\vect$ according to \eqref{eq:quantization}.
\end{proposition}
Prop.~\ref{prop:general} applies to any continuous function defined on the probability simplex. In particular, it applies to information measures such as entropy and mutual information, which are continuous functions of the channel input pmf.
\subsection{Minimizing Relative Entropy}
Prop.~\ref{prop:general} is a qualitative result. It tells us that we can approximate a target pmf as close as desired, but it does not give the speed of convergence when $M$ increases, nor how to optimally quantize for a finite $M$. To get such results, we must specify a measure of approximation. One useful measure is the gap to capacity that results from using an $M$-type pmf instead of the capacity-achieving pmf. In \cite[Sec. IV.B]{abbe2011polar}, the authors derived a bound on this gap for AWGN channels when using $M$-type pmfs. However, the derivation depends heavily on having Gaussian noise. Getting similar results for general DIMCs seems difficult.

The relative entropy $\kl(\vecd\Vert\vect)$ of the channel input pmf $\vecd$ and the capacity-achieving pmf $\vect$ is an upper-bound on the gap to capacity that results from using $\vecd$ \cite[Sec. 3.4.3]{bocherer2012capacity}. Relative entropy is simpler to analyze than the exact gap to capacity since the (possibly complicated) structure of the channel enters only via the capacity-achieving pmf. We will therefore address question Q1 (rate of convergence) and question Q2 (optimal $M$-type pmf) with respect to $\kl(\vecd\Vert\vect)$.
%
%
%
%
\section{Convergence Rate}
\label{sec:convergence}
The relative entropy achieved by the $M$-type pmf $\vecd$ obtained by quantizing $\vect$  according to \eqref{eq:quantization} is bounded as
\begin{align}
\kl(\vecd\Vert\vect)&=\sum_{i\colon d_i>0} d_i\log\frac{d_i}{t_i}\\
&\overset{\text{(a)}}{\leq} \sum_{i\colon d_i>0} d_i\log\frac{t_i+\frac{1}{M}}{t_i}\\
&= \sum_{i\colon d_i>0} d_i\log\Bigl(1+\frac{1}{Mt_i}\Bigr)\\
&\overset{\text{(b)}}{\leq} \sum_{i\colon d_i>0} d_i\frac{1}{Mt_i}\\
&\overset{\text{(c)}}{\leq} \sum_{i\colon d_i>0} d_i\frac{1}{\displaystyle M\min_{j\colon t_j>0}t_j}\\
&= \frac{1}{\displaystyle \min_{j\colon t_j>0}t_j}\cdot\frac{1}{M}.
\end{align}
where (a) follows by \eqref{eq:quantBounds}, (b) follows by \text{$\log(1+x)\leq x$}, and where (c) follows by \eqref{eq:probZero}. Thus we have the following result.
\begin{proposition}\label{prop:rate}
For each target pmf $\vect$ there exists a constant $T>0$ such that
\begin{align}
\kl(\vecd_M\Vert\vect)\leq T/M,\quad\forall M\geq 1
\end{align}
where $\vecd_M$ is the $M$-type pmf obtained by quantizing $\vect$ according to \eqref{eq:quantization}.
\end{proposition}








